Building Statistical Shape Spaces for 3D Human Modeling

Statistical models of 3D human shape and pose learned from scan databases have developed into valuable tools to solve a variety of vision and graphics problems. Unfortunately, most publicly available models are of limited expressiveness as they were learned on very small databases that hardly reflect the true variety in human body shapes. In this paper, we contribute by rebuilding a widely used statistical body representation from the largest commercially available scan database, and making the resulting model available to the community (visit http://humanshape.mpi-inf.mpg.de). As preprocessing several thousand scans for learning the model is a challenge in itself, we contribute by developing robust best practice solutions for scan alignment that quantitatively lead to the best learned models. We make implementations of these preprocessing steps also publicly available. We extensively evaluate the improved accuracy and generality of our new model, and show its improved performance for human body reconstruction from sparse input data.

==> figure_bootstrap_fit.tex <==
\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 1.5pt
\renewcommand{\arraystretch}{0.2}
\subfigure[scan]{
\includegraphics[trim=6cm 1cm 6cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-scanidx-1-thresh1-0-thresh2-10-scan-45.png}
}
%hspace{0.5em}
\subfigure[iteration 0]{
\includegraphics[trim=6cm 1cm 6cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-scanidx-1-thresh1-0-thresh2-10-meanDist-45.png}
}
%\hspace{0.5em}
\subfigure[iteration 2]{
\includegraphics[trim=6cm 1cm 6cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-2-scanidx-1-thresh1-0-thresh2-10-meanDist-45.png}
}
%\hspace{0.5em}
\subfigure[iteration 4]{
\includegraphics[trim=6cm 1cm 6cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-scanidx-1-thresh1-0-thresh2-10-meanDist-45.png}
}

\caption{Scan (a) and sample fitting results after zero (b), two (c),
  and four (d) bootstrapping iterations when using the model of Jain
  et al.~\cite{Jain:2010:MovieReshape} as initialization for iteration
  0. 
  %The human scan (green) is overlaid with the deformed template(red).
}
  \label{fig:boots-fit-ex}
\egroup
\end{figure*}

% \begin{figure*}[tbp]
% \centering
% \bgroup
% \tabcolsep 1.5pt
% \renewcommand{\arraystretch}{0.2}
% \subfigure[scan]{
% \begin{tabular}{cc}
% \includegraphics[trim=7cm 1cm 6cm 1cm,clip=true,height=0.2\linewidth]{scan-CSR0001A--45.png}&
% \includegraphics[trim=9cm 1cm 5cm 1cm,clip=true,height=0.2\linewidth]{scan-CSR0001A-45.png}\\
% \end{tabular}
% }
% %hspace{0.5em}
% \subfigure[iteration 0]{
% \begin{tabular}{cc}
% \includegraphics[trim=7cm 1cm 6cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-CSR0001A--45.png}&
% \includegraphics[trim=9cm 1cm 5cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-CSR0001A-45.png}\\
% \end{tabular}
% }
% %\hspace{0.5em}
% \subfigure[iteration 2]{
% \begin{tabular}{cc}
% \includegraphics[trim=7cm 1cm 6cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-2-CSR0001A--45.png}&
% \includegraphics[trim=9cm 1cm 5cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-2-CSR0001A-45.png}\\
% \end{tabular}
% }
% %\hspace{0.5em}
% \subfigure[iteration 4]{
% \begin{tabular}{cc}
% \includegraphics[trim=7cm 1cm 6cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-CSR0001A--45.png}&
% \includegraphics[trim=9cm 1cm 5cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-CSR0001A-45.png}\\
% \end{tabular}
% }

% \caption{Scan (a) and sample fitting results after zero (b), two (c), and four (d) bootstrapping iterations when using the model of Jain et al.~\cite{Jain:2010:MovieReshape} as initialization for iteration 0. The human scan (green) is overlaid with the deformed template (red).}
%   \label{fig:boots-fit-ex}
% \egroup
% \end{figure*}

==> figure_caesar_eval_all_dist_scan.tex <==
\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 1.5pt
\renewcommand{\arraystretch}{0.2}

\begin{tabular}{ccccc}
\# train &\multicolumn{4}{c}{\# PCA coefficients}\\
 sampl. &\\

  & 20 & 30 & 40 & 50 \\
\begin{sideways} \quad\quad\quad\quad\quad all \end{sideways}
&
\includegraphics[width=0.24\linewidth]{caesar-test-nPCA-20-0-20.pdf}
&
\includegraphics[width=0.24\linewidth]{caesar-test-nPCA-30-0-20.pdf}
&
\includegraphics[width=0.24\linewidth]{caesar-test-nPCA-40-0-20.pdf}
&
\includegraphics[width=0.24\linewidth]{caesar-test-nPCA-50-0-20.pdf}
\\[2pt]
\end{tabular}
\caption{Fitting error on the subset of 14 scans from ``CAESAR''
  dataset by Hasler et al. \cite{HaslerBM2009} and our proposed
  models. Shown is proportion of vertices [\%] which fitting error
  falls below a certain threshold.}
\egroup
\end{figure*}

==> figure_caesar_eval_avg_dist.tex <==
\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 0.0pt
\renewcommand{\arraystretch}{0.0}
\subfigure[Total fitting error]{
\begin{tabular}{c}
\includegraphics[height=0.20\linewidth]{caesar-test-nPCA-20-0-20.pdf}\\
\\
\vspace{0.8em}
\end{tabular}
}
\hspace{3em}
\subfigure[Mean fitting error]{
\begin{tabular}{ccccc}
\includegraphics[trim=0cm 0cm 5cm 0cm, clip=true,
height=0.20\linewidth]{model-mpii-corrected-scans-test-nPCA-20-thresh1-0-thresh2-10-meanDist-45.pdf}
&\quad
\includegraphics[trim=0cm 0cm 5cm 0cm, clip=true,
height=0.20\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-test-nPCA-20-thresh1-0-thresh2-10-meanDist-45.pdf}
&\quad
\includegraphics[trim=0cm 0cm 5cm 0cm, clip=true,
height=0.20\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-test-nPCA-20-thresh1-0-thresh2-10-meanDist-45.pdf}
&\quad
\includegraphics[trim=0cm 0cm 5cm 0cm, clip=true,
height=0.20\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-test-nPCA-20-thresh1-0-thresh2-10-meanDist-45.pdf}\\[2pt]
\footnotesize \hasler \cite{HaslerBM2009}& \quad\footnotesize \oursFive
&\quad\footnotesize \oursFiveWSX & \quad\footnotesize \oursFiveNH\\
%& &\quad\footnotesize + norm WSX& \quad\footnotesize + norm NH\\
\vspace{0.5em}
\end{tabular}
}
\caption{Fitting error on the subset of 14 scans from ``CAESAR''
  dataset by Hasler et al. \cite{HaslerBM2009} and our proposed
  models. Shown are (a) proportion of vertices [\%] which fitting
  error falls below a certain threshold and (b) average fitting error
  per vertex.}
  \label{fig:init-avg-dist}
\egroup
\end{figure*}

==> figure_init_all_dist.tex <==
%% \renewcommand{\subfigtopskip}{0pt}%
%% \renewcommand{\subfigcapskip}{5pt}%
%% \renewcommand{\subfigbottomskip}{15pt}% 
%% \renewcommand{\subfigcapmargin}{0pt}%
\begin{figure}[tbp]
\centering
\bgroup
\tabcolsep 1.5pt
\renewcommand{\arraystretch}{0.2}
\includegraphics[width=1.0\linewidth]{init-nrd-all-dist.pdf}
\caption{Proportion of vertices [\%] which fitting error falls below a
  certain threshold.}
  \label{fig:init-all-dist}
\egroup
\end{figure}


==> figure_kinect.tex <==
\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 0.0pt
\renewcommand{\arraystretch}{0.0}

\subfigure[\footnotesize scan]{
\begin{tabular}{ccc}
\begin{sideways} \bf \quad\quad Female 1 front \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-1-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\begin{sideways} \bf \quad\quad Female 1 back \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-2-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\begin{sideways} \bf \quad\quad Female 2 front \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-3-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\begin{sideways} \bf \quad\quad Female 2 back \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-4-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\begin{sideways} \bf \quad\quad Female 3 front \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-5-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\begin{sideways} \bf \quad\quad Female 3 back \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-6-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\hspace{1.8em}
\subfigure[\footnotesize Hasler et al.]{
\begin{tabular}{c}
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-ankle-scanidx-2-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-ankle-scanidx-3-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-ankle-scanidx-4-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-ankle-scanidx-5-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-ankle-scanidx-6-thresh1-0-thresh2-20-meanDist-45.pdf}\\

\end{tabular}
}
\hspace{1.8em}
\subfigure[\footnotesize ours 4 iter]{
\begin{tabular}{c}
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-2-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-3-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-4-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-5-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-6-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\hspace{1.8em}
\subfigure[\footnotesize ours 4 iter + norm WSX]{
\begin{tabular}{c}
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-WSX-no-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-WSX-no-ankle-scanidx-2-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-WSX-no-ankle-scanidx-3-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-WSX-no-ankle-scanidx-4-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-WSX-no-ankle-scanidx-5-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-WSX-no-ankle-scanidx-6-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\hspace{1.8em}
\subfigure[\footnotesize ours 4 iter + norm NH]{
\begin{tabular}{c}
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-NH-no-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-NH-no-ankle-scanidx-2-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-NH-no-ankle-scanidx-3-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-NH-no-ankle-scanidx-4-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-NH-no-ankle-scanidx-5-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-NH-no-ankle-scanidx-6-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}

\caption{\todo{}.}
  \label{fig:init-mean-dist}
\egroup
\end{figure*}

==> figure_kinect_all_dist.tex <==
% \begin{figure*}[tbp]
% \centering
% \bgroup
% \tabcolsep 1.5pt
% \renewcommand{\arraystretch}{0.2}
% \subfigure[Total fitting error]{
% \begin{tabular}{c}
% \includegraphics[height=0.2\linewidth]{bootstrap-all-dist.pdf}\\
% \\
% \vspace{0.8em}
% \end{tabular}
% }
% \subfigure[Mean fitting error]{
% \begin{tabular}{ccc}
% \includegraphics[height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-meanDist.pdf}&\quad\quad
% \includegraphics[height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-2-meanDist.pdf}&\quad\quad
% %\includegraphics[height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-3-meanDist.pdf}&\quad\quad
% \includegraphics[height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-meanDist.pdf}\\
% init-NRD 3&init-NRD 3 boots 2&init-NRD 3 boots 4\\
% \vspace{0.5em}
% \end{tabular}
% }

% \caption{Fitting error after a single (init-NRD 3), three (bootsrap 2)
%   and five (bootstrap 4) passes through ``CAESAR'' database. Shown
%   are (a) proportion of vertices [\%] which fitting error falls below
%   a certain threshold and (b) average fitting error per
%   vertex.}
%   \label{fig:init-mean-dist}
% \egroup
% \end{figure*}

\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 1.5pt
\renewcommand{\arraystretch}{0.2}
% \subfigure[5 PCA coefficients]{
% \begin{tabular}{c}
% \includegraphics[width=0.22\linewidth]{kinect-no-ankle-nPCA-5-0-20.pdf}\\
% \vspace{0.7em}
% \end{tabular}
% }
% \subfigure[10 PCA coefficients]{
% \begin{tabular}{c}
% \includegraphics[width=0.22\linewidth]{kinect-no-ankle-nPCA-10-0-20.pdf}\\
% \vspace{0.7em}
% \end{tabular}
% }
% \subfigure[15 PCA coefficients]{
% \begin{tabular}{c}
% \includegraphics[width=0.22\linewidth]{kinect-no-ankle-nPCA-15-0-20.pdf}\\
% \vspace{0.7em}
% \end{tabular}
% }
% \subfigure[20 PCA coefficients]{
% \begin{tabular}{c}
% \includegraphics[width=0.22\linewidth]{kinect-no-ankle-nPCA-15-0-20.pdf}\\
% \vspace{0.7em}
% \end{tabular}
% }
\subfigure[Low errors (0 - 10 mm)]{
\begin{tabular}{c}
\includegraphics[width=0.22\linewidth]{kinect-no-hip-sho-tho-ankle-0-10.pdf}\\
\vspace{0.7em}
\end{tabular}
}
\subfigure[High errors (10 - 50 mm)]{
\begin{tabular}{c}
\includegraphics[width=0.22\linewidth]{kinect-no-hip-sho-tho-ankle-10-50.pdf}\\
\vspace{0.7em}
\end{tabular}
}
\subfigure[Low errors (0 - 10 mm)]{
\begin{tabular}{c}
\includegraphics[width=0.22\linewidth]{kinect-no-hip-sho-tho-ankle-semih-0-10.pdf}\\
\vspace{0.7em}
\end{tabular}
}
\subfigure[High errors (10 - 50 mm)]{
\begin{tabular}{c}
\includegraphics[width=0.22\linewidth]{kinect-no-hip-sho-tho-ankle-semih-10-50.pdf}\\
\vspace{0.7em}
\end{tabular}
}
\caption{Fitting error on the Kinect scans \cite{HeltenPAE13} by
  Hasler et al. \cite{HaslerBM2009} and our proposed models. Shown is
  proportion of vertices [\%] which fitting error falls below a
  certain threshold in low error (a) and (b) high error regimes.}
\egroup
\end{figure*}

==> figure_kinect_male.tex <==
\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 0.0pt
\renewcommand{\arraystretch}{0.0}
% \subfigure[\footnotesize scan]{
% \begin{tabular}{cc}
% \includegraphics[height=0.14\linewidth]{kinect-scanidx-1-scan.pdf}&
% \includegraphics[height=0.14\linewidth]{kinect-scanidx-2-scan.pdf}\\
% \end{tabular}
% }
% \subfigure[\footnotesize Hasler et al.]{
% \begin{tabular}{cc}
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-mpii-scanidx-1-thresh1-0-thresh2-20-meanDist.pdf}&
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-mpii-scanidx-2-thresh1-0-thresh2-20-meanDist.pdf}\\
% \end{tabular}
% }
% \subfigure[\footnotesize ours 4 iter]{
% \begin{tabular}{cc}
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-scanidx-1-thresh1-0-thresh2-20-meanDist.pdf}&
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-scanidx-2-thresh1-0-thresh2-20-meanDist.pdf}\\
% \end{tabular}
% }
% \subfigure[\footnotesize ours 4 iter + norm WSX]{
% \begin{tabular}{cc}
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-norm-WSX-scanidx-1-thresh1-0-thresh2-20-meanDist.pdf}&
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-norm-WSX-scanidx-2-thresh1-0-thresh2-20-meanDist.pdf}\\
% \end{tabular}
% }
% \subfigure[\footnotesize ours 4 iter + norm NH]{
% \begin{tabular}{cc}
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-norm-NH-scanidx-1-thresh1-0-thresh2-20-meanDist.pdf}&
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-norm-NH-scanidx-2-thresh1-0-thresh2-20-meanDist.pdf}\\
% \end{tabular}
% }

\subfigure[\footnotesize scan]{
\begin{tabular}{ccc}
\begin{sideways} \bf \quad\quad\quad Male 1 front \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-7-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-7-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\begin{sideways} \bf \quad\quad\quad Male 1 back \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-8-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-7-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\begin{sideways} \bf \quad\quad\quad Male 2 front \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-9-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-7-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\begin{sideways} \bf \quad\quad\quad Male 2 back \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-10-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-7-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\begin{sideways} \bf \quad\quad\quad Male 3 front \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-11-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-7-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\begin{sideways} \bf \quad\quad\quad Male 3 back \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-12-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-7-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\hspace{1.8em}
\subfigure[\footnotesize Hasler et al.]{
\begin{tabular}{c}
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-ankle-scanidx-7-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-ankle-scanidx-8-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-ankle-scanidx-9-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-ankle-scanidx-10-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-ankle-scanidx-11-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-ankle-scanidx-12-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\hspace{1.8em}
\subfigure[\footnotesize ours 4 iter]{
\begin{tabular}{c}
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-7-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-8-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-9-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-10-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-11-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-12-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\hspace{1.8em}
\subfigure[\footnotesize ours 4 iter + norm WSX]{
\begin{tabular}{c}
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-WSX-no-ankle-scanidx-7-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-WSX-no-ankle-scanidx-8-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-WSX-no-ankle-scanidx-9-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-WSX-no-ankle-scanidx-10-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-WSX-no-ankle-scanidx-11-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-WSX-no-ankle-scanidx-12-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\hspace{1.8em}
\subfigure[\footnotesize ours 4 iter + norm NH]{
\begin{tabular}{c}
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-NH-no-ankle-scanidx-7-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-NH-no-ankle-scanidx-8-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-NH-no-ankle-scanidx-9-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-NH-no-ankle-scanidx-10-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-NH-no-ankle-scanidx-11-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-norm-NH-no-ankle-scanidx-12-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\caption{\todo{}}
  \label{fig:init-mean-dist}
\egroup
\end{figure*}

==> figure_kinect_pose.tex <==
\begin{figure*}[t]
\centering
\bgroup
\tabcolsep 10.0pt
\renewcommand{\arraystretch}{0.0}

\subfigure[\footnotesize front/back depth scans]{
\begin{tabular}{cccc}
\begin{sideways} \bf \quad\quad Female 1 \end{sideways}&\quad
\includegraphics[height=0.15\linewidth]{F1_front00.png}&
\includegraphics[height=0.15\linewidth]{F1_back00.png}&
% \includegraphics[height=0.20\linewidth]{kinect-scanidx-1-scan-45.pdf}&
% \includegraphics[height=0.20\linewidth]{kinect-scanidx-2-scan-45.pdf}&
%\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.15\linewidth]{kinect-mpii-no-hip-sho-tho-ankle-scan-new-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\

% \begin{sideways} \bf \quad\quad Female 2 \end{sideways}&\quad
% \includegraphics[height=0.17\linewidth]{F2_front00.png}&
% \includegraphics[height=0.17\linewidth]{F2_back00.png}&
% \includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \begin{sideways} \bf \quad\quad Female 3 \end{sideways}&\quad
% \includegraphics[height=0.17\linewidth]{F3_front00.png}&
% \includegraphics[height=0.17\linewidth]{F3_back00.png}&
% \includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\begin{sideways} \bf \quad\quad Male 1 \end{sideways}&\quad
\includegraphics[height=0.15\linewidth]{M1_front00.png}&
\includegraphics[height=0.15\linewidth]{M1_back00.png}&
%\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.15\linewidth]{kinect-mpii-no-hip-sho-tho-ankle-scan-new-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \begin{sideways} \bf \quad\quad Male 2 \end{sideways}&\quad
% \includegraphics[height=0.17\linewidth]{M2_front00.png}&
% \includegraphics[height=0.17\linewidth]{M2_back00.png}&
% \includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \begin{sideways} \bf \quad\quad Male 3 \end{sideways}&\quad
% \includegraphics[height=0.17\linewidth]{M3_front00.png}&
% \includegraphics[height=0.17\linewidth]{M3_back00.png}&
% \includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\hspace{1.0em}
\subfigure[\footnotesize \jain~\cite{Jain:2010:MovieReshape}]{
\begin{tabular}{c}
\includegraphics[trim=0cm 1.8cm 8.0cm 1.8cm,clip=true,height=0.15\linewidth]{kinect-mpii-no-hip-sho-tho-ankle-scan-new-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-hip-sho-tho-ankle-scan-new-scanidx-2-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-hip-sho-tho-ankle-scan-new-scanidx-3-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 1.8cm 8.0cm 1.8cm,clip=true,height=0.15\linewidth]{kinect-mpii-no-hip-sho-tho-ankle-scan-new-scanidx-4-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-hip-sho-tho-ankle-scan-new-scanidx-5-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-hip-sho-tho-ankle-scan-new-scanidx-6-thresh1-0-thresh2-20-meanDist-45.pdf}\\

\end{tabular}
}
\subfigure[\footnotesize \textit{ours}]{
\begin{tabular}{c}
\includegraphics[trim=0cm 1.8cm 8.0cm 1.8cm,clip=true,height=0.15\linewidth]{kinect-no-hip-sho-tho-ankle-scan-new-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-scan-new-scanidx-2-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-scan-new-scanidx-3-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 1.8cm 8.0cm 1.8cm,clip=true,height=0.15\linewidth]{kinect-no-hip-sho-tho-ankle-scan-new-scanidx-4-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-scan-new-scanidx-5-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-scan-new-scanidx-6-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\subfigure[\footnotesize \textit{ours + WSX}]{
\begin{tabular}{c}
\includegraphics[trim=0cm 1.8cm 8.0cm 1.8cm,clip=true,height=0.15\linewidth]{kinect-no-hip-sho-tho-ankle-norm-WSX-scan-new-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-norm-WSX-scan-new-scanidx-2-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-norm-WSX-scan-new-scanidx-3-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 1.8cm 8.0cm 1.8cm,clip=true,height=0.15\linewidth]{kinect-no-hip-sho-tho-ankle-norm-WSX-scan-new-scanidx-4-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-norm-WSX-scan-new-scanidx-5-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-norm-WSX-scan-new-scanidx-6-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\hspace{1.0em}
\subfigure[\footnotesize \textit{ours + NH}]{
\begin{tabular}{c}
\includegraphics[trim=0cm 1.8cm 8.0cm 1.8cm,clip=true,height=0.15\linewidth]{kinect-no-hip-sho-tho-ankle-norm-NH-scan-new-scanidx-1-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-norm-NH-scan-new-scanidx-2-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-norm-NH-scan-new-scanidx-3-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 1.8cm 8.0cm 1.8cm,clip=true,height=0.15\linewidth]{kinect-no-hip-sho-tho-ankle-norm-NH-scan-new-scanidx-4-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-norm-NH-scan-new-scanidx-5-thresh1-0-thresh2-20-meanDist-45.pdf}\\
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-norm-NH-scan-new-scanidx-6-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}

\caption{Per-vertex shape fitting error (mm) of multiple methods on sample individuals of Helten et al.~\cite{HeltenPAE13}.}
  \label{fig:kinect-pose}
\egroup
\end{figure*}

==> figure_kinect_semih.tex <==
\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 0.0pt
\renewcommand{\arraystretch}{0.0}
% \subfigure[\footnotesize scan]{
% \begin{tabular}{cc}
% \includegraphics[height=0.14\linewidth]{kinect-scanidx-1-scan.pdf}&
% \includegraphics[height=0.14\linewidth]{kinect-scanidx-2-scan.pdf}\\
% \end{tabular}
% }
% \subfigure[\footnotesize Hasler et al.]{
% \begin{tabular}{cc}
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-mpii-scanidx-1-thresh1-0-thresh2-20-meanDist.pdf}&
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-mpii-scanidx-2-thresh1-0-thresh2-20-meanDist.pdf}\\
% \end{tabular}
% }
% \subfigure[\footnotesize ours 4 iter]{
% \begin{tabular}{cc}
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-scanidx-1-thresh1-0-thresh2-20-meanDist.pdf}&
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-scanidx-2-thresh1-0-thresh2-20-meanDist.pdf}\\
% \end{tabular}
% }
% \subfigure[\footnotesize ours 4 iter + norm WSX]{
% \begin{tabular}{cc}
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-norm-WSX-scanidx-1-thresh1-0-thresh2-20-meanDist.pdf}&
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-norm-WSX-scanidx-2-thresh1-0-thresh2-20-meanDist.pdf}\\
% \end{tabular}
% }
% \subfigure[\footnotesize ours 4 iter + norm NH]{
% \begin{tabular}{cc}
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-norm-NH-scanidx-1-thresh1-0-thresh2-20-meanDist.pdf}&
% \includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.15\linewidth]{kinect-norm-NH-scanidx-2-thresh1-0-thresh2-20-meanDist.pdf}\\
% \end{tabular}
% }

\subfigure[\footnotesize scan]{
\begin{tabular}{ccc}
\begin{sideways} \bf \quad\quad\quad Male 1 front \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-13-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-7-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\begin{sideways} \bf \quad\quad\quad Male 1 back \end{sideways}&\quad
\includegraphics[height=0.20\linewidth]{kinect-scanidx-14-scan-45.pdf}&
\includegraphics[trim=10cm 0cm 0cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-ankle-scanidx-7-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\hspace{1.8em}
\subfigure[\footnotesize Hasler et al.]{
\begin{tabular}{c}
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-hip-sho-tho-ankle-scanidx-13-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-mpii-no-hip-sho-tho-ankle-scanidx-14-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\hspace{1.8em}
\subfigure[\footnotesize ours 4 iter]{
\begin{tabular}{c}
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-scanidx-13-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-scanidx-14-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\hspace{1.8em}
\subfigure[\footnotesize ours 4 iter + norm WSX]{
\begin{tabular}{c}
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-norm-WSX-scanidx-13-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-norm-WSX-scanidx-14-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\hspace{1.8em}
\subfigure[\footnotesize ours 4 iter + norm NH]{
\begin{tabular}{c}
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-norm-NH-scanidx-13-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\includegraphics[trim=0cm 0cm 4.8cm 0cm,clip=true,height=0.20\linewidth]{kinect-no-hip-sho-tho-ankle-norm-NH-scanidx-14-thresh1-0-thresh2-20-meanDist-45.pdf}\\
\end{tabular}
}
\caption{\todo{}}
  \label{fig:init-mean-dist}
\egroup
\end{figure*}

==> figure_kinect_seq_all_dist.tex <==
% \begin{figure*}[tbp]
% \centering
% \bgroup
% \tabcolsep 1.5pt
% \renewcommand{\arraystretch}{0.2}
% \subfigure[Total fitting error]{
% \begin{tabular}{c}
% \includegraphics[height=0.2\linewidth]{bootstrap-all-dist.pdf}\\
% \\
% \vspace{0.8em}
% \end{tabular}
% }
% \subfigure[Mean fitting error]{
% \begin{tabular}{ccc}
% \includegraphics[height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-meanDist.pdf}&\quad\quad
% \includegraphics[height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-2-meanDist.pdf}&\quad\quad
% %\includegraphics[height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-3-meanDist.pdf}&\quad\quad
% \includegraphics[height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-meanDist.pdf}\\
% init-NRD 3&init-NRD 3 boots 2&init-NRD 3 boots 4\\
% \vspace{0.5em}
% \end{tabular}
% }

% \caption{Fitting error after a single (init-NRD 3), three (bootsrap 2)
%   and five (bootstrap 4) passes through ``CAESAR'' database. Shown
%   are (a) proportion of vertices [\%] which fitting error falls below
%   a certain threshold and (b) average fitting error per
%   vertex.}
%   \label{fig:init-mean-dist}
% \egroup
% \end{figure*}

\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 1.5pt
\renewcommand{\arraystretch}{0.2}
\subfigure[Low errors (0 - 10 mm)]{
\begin{tabular}{c}
%\includegraphics[width=0.45\linewidth]{kinect-seq-no-ankle-0-10}\\
\includegraphics[width=0.45\linewidth]{kinect-seq-no-hip-sho-tho-ankle-0-10}\\
\vspace{0.7em}
\end{tabular}
}
\subfigure[High errors (10 - 50 mm)]{
\begin{tabular}{c}
%\includegraphics[width=0.45\linewidth]{kinect-seq-no-ankle-10-50}\\
\includegraphics[width=0.45\linewidth]{kinect-seq-no-hip-sho-tho-ankle-10-50}\\
\vspace{0.7em}
\end{tabular}
}
\caption{Fitting error on the Kinect scans \todo{cite CVIU} by
  Hasler et al. \cite{HaslerBM2009} and our proposed models. Shown is
  proportion of vertices [\%] which fitting error falls below a
  certain threshold in low error (a) and (b) high error regimes.}
\egroup
\end{figure*}

==> figure_kinect_seq_measurements.tex <==
% \begin{figure*}[tbp]
% \centering
% \bgroup
% \tabcolsep 1.5pt
% \renewcommand{\arraystretch}{0.2}
% \subfigure[Total fitting error]{
% \begin{tabular}{c}
% \includegraphics[height=0.2\linewidth]{bootstrap-all-dist.pdf}\\
% \\
% \vspace{0.8em}
% \end{tabular}
% }
% \subfigure[Mean fitting error]{
% \begin{tabular}{ccc}
% \includegraphics[height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-meanDist.pdf}&\quad\quad
% \includegraphics[height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-2-meanDist.pdf}&\quad\quad
% %\includegraphics[height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-3-meanDist.pdf}&\quad\quad
% \includegraphics[height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-meanDist.pdf}\\
% init-NRD 3&init-NRD 3 boots 2&init-NRD 3 boots 4\\
% \vspace{0.5em}
% \end{tabular}
% }

% \caption{Fitting error after a single (init-NRD 3), three (bootsrap 2)
%   and five (bootstrap 4) passes through ``CAESAR'' database. Shown
%   are (a) proportion of vertices [\%] which fitting error falls below
%   a certain threshold and (b) average fitting error per
%   vertex.}
%   \label{fig:init-mean-dist}
% \egroup
% \end{figure*}

\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 1.5pt
\renewcommand{\arraystretch}{0.2}
\begin{tabular}{ccc}
\includegraphics[width=0.3\linewidth]{kinect-seq-no-hip-sho-tho-ankle-measure-height.pdf}&
\includegraphics[width=0.3\linewidth]{kinect-seq-no-hip-sho-tho-ankle-measure-waist.pdf}&
\includegraphics[width=0.3\linewidth]{kinect-seq-no-hip-sho-tho-ankle-measure-chest.pdf}\\
\vspace{0.7em}
\end{tabular}

\caption{Measurement error on the Kinect scans \todo{cite CVIU} by
  Hasler et al. \cite{HaslerBM2009} and our proposed models.}
\egroup
\end{figure*}

==> figure_model_quality.tex <==
%% \renewcommand{\subfigtopskip}{0pt}%
%% \renewcommand{\subfigcapskip}{5pt}%
%% \renewcommand{\subfigbottomskip}{15pt}% 
%% \renewcommand{\subfigcapmargin}{0pt}%
\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 1.5pt
\renewcommand{\arraystretch}{0.2}
% \subfigure[Compactness]{\includegraphics[width=0.32\linewidth]{compactness-model-mpii-all-samples-warm-sched-3-bootstrap-4.pdf}}
% \subfigure[Generalization]{\includegraphics[width=0.32\linewidth]{generalization-model-mpii-all-samples-warm-sched-3-bootstrap-4.pdf}}
% \subfigure[Specificity]{\includegraphics[width=0.32\linewidth]{specificity-model-mpii-all-samples-warm-sched-3-bootstrap-4.pdf}}

% \subfigure[Compactness]{\includegraphics[width=0.32\linewidth]{compactness-model-mpii-all-samples-warm-sched-3-bootstrap-4-learn-all-scans-new.pdf}}
% \subfigure[Generalization]{\includegraphics[width=0.32\linewidth]{generalization-model-mpii-all-samples-warm-sched-3-bootstrap-4-learn-all-scans-new.pdf}}
% \subfigure[Specificity]{\includegraphics[width=0.32\linewidth]{specificity-model-mpii-all-samples-warm-sched-3-bootstrap-4-learn-all-scans-new.pdf}}
% \subfigure[absolute cumulative
% sum]{\includegraphics[width=0.32\linewidth]{compactness-model-mpii-all-samples-warm-sched-3-bootstrap-4-learn-all-scans-new-absolut.pdf}}

\subfigure[Generalization]{\includegraphics[width=0.32\linewidth]{generalization-model-mpii-all-samples-warm-sched-3-bootstrap-4-learn-all-scans-new-gt.pdf}}
\subfigure[Specificity]{\includegraphics[width=0.32\linewidth]{specificity-model-mpii-all-samples-warm-sched-3-bootstrap-4-learn-all-scans-new-gt.pdf}}
% \caption{Influence of bootstrapping on the quality of the learned
%   statistical shape model. Shown are (a) compactness, (b)
%   generalization and (c) specificity of the statistical model.}
%   \label{fig:model_eval_basic}
\caption{Influence of bootstrapping on the quality of the learned
  statistical shape model. Shown are (a) generalization and (b)
  specificity of the statistical model.}
  \label{fig:model_quality}
\egroup
\end{figure*}


==> figure_model_quality_pose_norm.tex <==
%% \renewcommand{\subfigtopskip}{0pt}%
%% \renewcommand{\subfigcapskip}{5pt}%
%% \renewcommand{\subfigbottomskip}{15pt}% 
%% \renewcommand{\subfigcapmargin}{0pt}%
\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 1.5pt
\renewcommand{\arraystretch}{0.2}
% \subfigure[Compactness]{\includegraphics[width=0.32\linewidth]{compactness-model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm.pdf}}
\subfigure[Generalization]{\includegraphics[width=0.32\linewidth]{generalization-model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm.pdf}}
\subfigure[Specificity]{\includegraphics[width=0.32\linewidth]{specificity-model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm.pdf}}

% \caption{Influence of pose normalization on the quality of the learned
%   statistical shape model. Shown are (a) compactness, (b)
%   generalization and (c) specificity of the statistical model when
%   using no normalization, computing normalization by
%   \cite{Neophytou2013} (NH) and \cite{WuhrerPIS12} (WSX).}
%   \label{fig:model_eval_basic}
\caption{Influence of pose normalization on the quality of the learned
  statistical shape model. Shown are (a)
  generalization and (b) specificity of the statistical model when
  using no normalization, computing normalization by
  \cite{Neophytou2013} (NH) and \cite{WuhrerPIS12} (WSX).}
  \label{fig:model_eval_basic}
\egroup
\end{figure*}


==> figure_model_quality_scans.tex <==
'%% \renewcommand{\subfigtopskip}{0pt}%
%% \renewcommand{\subfigcapskip}{5pt}%
%% \renewcommand{\subfigbottomskip}{15pt}% 
%% \renewcommand{\subfigcapmargin}{0pt}%
\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 1.5pt
\renewcommand{\arraystretch}{0.2}
% \subfigure[Compactness]{\includegraphics[width=0.32\linewidth]{compactness-model-mpii-all-samples-warm-sched-3-bootstrap-4-var-scans.pdf}}
% \subfigure[Generalization]{\includegraphics[width=0.32\linewidth]{generalization-model-mpii-all-samples-warm-sched-3-bootstrap-4-var-scans.pdf}}
% \subfigure[Specificity]{\includegraphics[width=0.32\linewidth]{specificity-model-mpii-all-samples-warm-sched-3-bootstrap-4-var-scans.pdf}}\\
% \subfigure[Compactness]{\includegraphics[width=0.32\linewidth]{compactness-model-mpii-all-samples-warm-sched-3-bootstrap-4-var-scans.pdf}}
\subfigure[Generalization]{\includegraphics[width=0.32\linewidth]{generalization-model-mpii-all-samples-warm-sched-3-bootstrap-4-test-all.pdf}}
\subfigure[Specificity]{\includegraphics[width=0.32\linewidth]{specificity-model-mpii-all-samples-warm-sched-3-bootstrap-4-test-all.pdf}}

% \caption{Influence of the number of training samples on the quality of
%   the learned statistical shape model. Shown are (a) compactness, (b)
%   generalization and (c) specificity of the statistical model.}
\caption{Influence of the number of training samples on the quality of
  the learned statistical shape model. Shown are (a)
  generalization and (b) specificity of the statistical model.}

  \label{fig:model-quality-scans}
\egroup
\end{figure*}


==> figure_model_var.tex <==
\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 1.5pt
\renewcommand{\arraystretch}{0.2}
\subfigure[scan]{
\begin{tabular}{cc}
\includegraphics[trim=7cm 1cm 6cm 1cm,clip=true,height=0.2\linewidth]{scan-CSR0001A--45.png}&
\includegraphics[trim=9cm 1cm 5cm 1cm,clip=true,height=0.2\linewidth]{scan-CSR0001A-45.png}\\
\end{tabular}
}
%hspace{0.5em}
\subfigure[init-NRD 3]{
\begin{tabular}{cc}
\includegraphics[trim=7cm 1cm 6cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-CSR0001A--45.png}&
\includegraphics[trim=9cm 1cm 5cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-CSR0001A-45.png}\\
\end{tabular}
}
%\hspace{0.5em}
\subfigure[init-NRD 3 boots 2]{
\begin{tabular}{cc}
\includegraphics[trim=7cm 1cm 6cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-2-CSR0001A--45.png}&
\includegraphics[trim=9cm 1cm 5cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-2-CSR0001A-45.png}\\
\end{tabular}
}
%\hspace{0.5em}
\subfigure[init-NRD 3 boots 4]{
\begin{tabular}{cc}
\includegraphics[trim=7cm 1cm 6cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-CSR0001A--45.png}&
\includegraphics[trim=9cm 1cm 5cm 1cm,clip=true,height=0.2\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-CSR0001A-45.png}\\
\end{tabular}
}

\caption{Sample fitting results after (b) single (init-NRD 3), (c)
  three (bootsrap 2) and (d) five (bootstrap 4) passes through
  ``CAESAR'' database. Human scan (green) is overlaid with the
  deformed template (red).}
  \label{fig:init-mean-dist}
\egroup
\end{figure*}

==> figure_pca_components.tex <==
%% \renewcommand{\subfigtopskip}{0pt}%
%% \renewcommand{\subfigcapskip}{5pt}%
%% \renewcommand{\subfigbottomskip}{15pt}% 
%% \renewcommand{\subfigcapmargin}{0pt}%
\newcommand\h{0.20}

\begin{figure*}[tbp]
\centering
\bgroup
\tabcolsep 0.1pt
\renewcommand{\arraystretch}{0.0}
\begin{tabular}{c cc c cc c cc c cc c cc c cc c cc c cc c cc c cc c cc}
\begin{sideways} \bf \textit \quad\quad \jain~\cite{Jain:2010:MovieReshape} \end{sideways}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-1--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-1-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-2-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-2--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-3-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-3--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-4-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-4--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-5-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-5--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-6-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-6--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-7-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-7--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-8-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-8--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-9-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-9--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-10-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-corrected-scans-idxShape-10--1-vp-90.png}\\[-5pt]
\begin{sideways} \bf \textit \quad\quad\quad CAESAR \end{sideways}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-1-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-1--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-2-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-2--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-3--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-3-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-4--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-4-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-5-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-5--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-6--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-6-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-7--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-7-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-8--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-8-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-9--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-9-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-10--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-idxShape-10-1-vp-90.png}\\[-5pt]
\begin{sideways} \quad\bf \textit CAESAR + \WSX \end{sideways}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-1-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-1--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-2-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-2--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-3-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-3--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-4-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-4--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-5--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-5-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-6--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-6-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-7--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-7-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-8--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-8-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-9--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-9-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-10--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-wuhrer-norm-idxShape-10-1-vp-90.png}\\[-5pt]

\begin{sideways}\quad \bf \textit CAESAR + \NH \end{sideways}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-1-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-1--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-2-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-2--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-3-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-3--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-4-1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-4--1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-5--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-5-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-6--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-6-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-7--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-7-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-8--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-8-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-9--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-9-1-vp-90.png}&
\quad\quad&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-10--1-vp-90.png}&
\includegraphics[trim=9.0cm 1cm 8.7cm 1cm, clip=true, height=\h\linewidth]{model-mpii-all-samples-warm-sched-3-bootstrap-4-hilton-norm-idxShape-10-1-vp-90.png}\\
\bf st. dev.&
$+3 \sigma$& $-3 \sigma$&&
$+3 \sigma$& $-3 \sigma$&&
$+3 \sigma$& $-3 \sigma$&&
$+3 \sigma$& $-3 \sigma$&&
$+3 \sigma$& $-3 \sigma$&&
$+3 \sigma$& $-3 \sigma$&&
$+3 \sigma$& $-3 \sigma$&&
$+3 \sigma$& $-3 \sigma$&&
$+3 \sigma$& $-3 \sigma$&&
$+3 \sigma$& $-3 \sigma$\\

\bf PCA id&
\multicolumn{2}{c}{I}&&
\multicolumn{2}{c}{II}&&
\multicolumn{2}{c}{III}&&
\multicolumn{2}{c}{IV}&&
\multicolumn{2}{c}{V}&&
\multicolumn{2}{c}{VI}&&
\multicolumn{2}{c}{VII}&&
\multicolumn{2}{c}{VIII}&&
\multicolumn{2}{c}{IX}&&
\multicolumn{2}{c}{X}\\

\end{tabular}
\caption{Visualization of the first five PCA eigenvectors scaled by
  $\pm3 \sigma$ (standard deviation). Shown are eigenvectors of the
  simplified SCAPE space by Jain et al.~\cite{Jain:2010:MovieReshape}
  (row 1) and the simplified SCAPE spaces trained using our processed
  data without (row 2) and with posture normalization
  using \WSX~\cite{WuhrerPIS12} (row 3) and \NH~\cite{Neophytou2013}
  (row 4).}
  \label{fig:model_vis_pca}
\egroup
\end{figure*}


==> table_datagen_parse.tex <==
\tabcolsep 5pt
\begin{table}[tbp]
\normalsize
  \centering
  \begin{tabular}{@{} l ccc @{}}
    \toprule
    Model & range&\multicolumn{2}{c}{sampling}     \\
    & $\pm \sigma$ & uniform&normal\\
    \toprule

Hasler et al. & 4.0& 85.9 & 87.0\\
ours 5 iter & 4.0& 83.4 & 84.8\\
ours 5 iter + norm WSX & 4.0&81.9 & 79.3\\
ours 5 iter + norm NH & 4.0 & 85.2 & 81.0\\
Hasler et al. & 3.0& 86.6 & 86.2\\
ours 5 iter & 3.0&  87.6 &81.3\\
ours 5 iter + norm WSX & 3.0& 87.0 &86.7\\
ours 5 iter + norm NH & 3.0&  80.9 & 80.7\\
Hasler et al. & 2.0&  84.5 & 85.7\\
ours 5 iter & 2.0&  85.3 & 80.8\\
ours 5 iter + norm WSX & 2.0& 82.9 & 86.4\\
ours 5 iter + norm NH & 2.0 & 83.7 & 79.6\\
Hasler et al. & 1.0& 83.3 & 86.9\\
ours 5 iter & 1.0& 84.8 & 84.9\\
ours 5 iter + norm WSX & 1.0&  84.8 & 82.9\\
ours 5 iter + norm NH & 1.0& 80.2 & 82.3\\


% Hasler et al. & 4.0& gauss & 87.0 \\
% ours 4 iter & 4.0& gauss & 84.8 \\
% ours 4 iter + norm WSX & 4.0& gauss & 79.3 \\
% ours 4 iter + norm NH & 4.0& gauss & 81.0 \\
% Hasler et al. & 3.0& gauss & 86.2 \\
% ours 4 iter & 3.0& gauss & 81.3 \\
% ours 4 iter + norm WSX & 3.0& gauss & 86.7 \\
% ours 4 iter + norm NH & 3.0& gauss & 80.7 \\
% Hasler et al. & 2.0& gauss & 85.7 \\
% ours 4 iter & 2.0& gauss & 80.8 \\
% ours 4 iter + norm WSX & 2.0& gauss & 86.4 \\
% ours 4 iter + norm NH & 2.0& gauss & 79.6 \\
% Hasler et al. & 1.0& gauss & 86.9 \\
% ours 4 iter & 1.0& gauss & 84.9 \\
% ours 4 iter + norm WSX & 1.0& gauss & 82.9 \\
% ours 4 iter + norm NH & 1.0& gauss & 82.3 \\
% Hasler et al. & 4.0& uniform & 85.9 \\
% ours 4 iter & 4.0& uniform & 83.4 \\
% ours 4 iter + norm WSX & 4.0& uniform & 81.9 \\
% ours 4 iter + norm NH & 4.0& uniform & 85.2 \\
% Hasler et al. & 3.0& uniform & 86.6 \\
% ours 4 iter & 3.0& uniform & 87.6 \\
% ours 4 iter + norm WSX & 3.0& uniform & 87.0 \\
% ours 4 iter + norm NH & 3.0& uniform & 80.9 \\
% Hasler et al. & 2.0& uniform & 84.5 \\
% ours 4 iter & 2.0& uniform & 85.3 \\
% ours 4 iter + norm WSX & 2.0& uniform & 82.9 \\
% ours 4 iter + norm NH & 2.0& uniform & 83.7 \\
% Hasler et al. & 1.0& uniform & 83.3 \\
% ours 4 iter & 1.0& uniform & 84.8 \\
% ours 4 iter + norm WSX & 1.0& uniform & 84.8 \\
% ours 4 iter + norm NH & 1.0& uniform & 80.2 \\

\midrule
Hasler et al. (CVPR'12) & 4.0&  85.4 & 90.1 \\

\bottomrule
\end{tabular}
  \caption{\todo{}DPM detector, ``Parse'' dataset.}
  \label{tab:dpm-num-samples}
\end{table}


==> table_datagen_parse_channels.tex <==
\tabcolsep 5pt
\begin{table}[tbp]
  \normalsize
  \centering
  \begin{tabular}{@{} l ccc @{}}
    \toprule
    Model & range&\multicolumn{2}{c}{sampling}     \\
    & $\pm \sigma$ & uniform&normal\\
    \toprule
    
    Hasler et al. & 4.0& - & 40.3\\
    ours 4 iter & 4.0& - & 37.5\\
    ours 4 iter + norm WSX & 4.0&- & 44.9\\
    ours 4 iter + norm NH & 4.0 & - & 34.8\\

\midrule
Hasler et al. (CVPR'12) & 4.0&  85.4 & 90.1 \\

\bottomrule
\end{tabular}
  \caption{\todo{}Shan-Shan channels detector, ``Parse'' dataset.}
  \label{tab:dpm-num-samples}
\end{table}


==> table_datagen_parse_mean.tex <==
\tabcolsep 1pt
\begin{table}[tbp]
  \normalsize
  \centering
  \begin{tabular}{@{} l ccccc @{}}
    \toprule
    Model & range&\multicolumn{4}{c}{sampling}     \\
    & $\pm \sigma$ & \multicolumn{2}{c}{uniform}&\multicolumn{2}{c}{normal}\\
    &              & mean & st.d. &mean & st.d. \\
    \toprule
    Hasler et al. & 4.0 & 86.1 & 2.0 & 85.6 & 1.8 \\
    Hasler et al. & 3.0 & 85.6 & 2.0 & 85.1 & 1.6 \\
    Hasler et al. & 2.0 & 84.3 & 1.7 & 84.9 & 1.1 \\
    Hasler et al. & 1.0 & 85.4 & 2.3 & 85.0 & 1.3 \\
    ours 5 iter & 4.0 & 86.1 & 2.3 & 85.6 & 1.0 \\
    ours 5 iter & 3.0 & 85.1 & 1.9 & 85.2 & 1.7 \\
    ours 5 iter & 2.0 & 84.0 & 2.4 & 84.7 & 1.3 \\
    ours 5 iter & 1.0 & 82.1 & 2.6 & 83.1 & 2.2 \\
    ours 5 iter + norm WSX & 4.0 & 85.5 & 1.4 & 84.8 & 1.1 \\
    ours 5 iter + norm WSX & 3.0 & 85.0 & 1.6 & 86.1 & 1.6 \\
    ours 5 iter + norm WSX & 2.0 & 85.4 & 1.4 & 84.9 & 2.1 \\
    ours 5 iter + norm WSX & 1.0 & 85.0 & 1.5 & 84.0 & 3.0 \\
    ours 5 iter + norm NH & 4.0 & 85.6 & 1.2 & 86.6 & 1.6 \\
    ours 5 iter + norm NH & 3.0 & 85.3 & 1.6 & 84.9 & 1.9 \\
    ours 5 iter + norm NH & 2.0 & 83.9 & 1.6 & 84.4 & 2.3 \\
    ours 5 iter + norm NH & 1.0 & 82.6 & 3.9 & 84.3 & 1.7 \\
%\midrule
%Hasler et al. (CVPR'12) & 4.0&  85.4 & 90.1 \\

\bottomrule
\end{tabular}
  \caption{\todo{}DPM detector, ``Parse'' dataset.}
  \label{tab:dpm-num-samples}
\end{table}

